Orbit-finite linear programming

An infinite set is orbit-finite if, up to permutations of the underlying structure of atoms, it has only finitely many elements. We study a generalisation of linear programming where constraints are expressed by an orbit-finite system of linear inequalities. As our principal contribution we provide a decision procedure for checking if such a system has a real solution, and for computing the minimal/maximal value of a linear objective function over the solution set. We also show undecidability of these problems in case when only integer solutions are considered. Therefore orbit-finite linear programming is decidable, while orbit-finite integer linear programming is not.

==> Makefile <==
TEX = pdflatex -shell-escape -interaction=nonstopmode -file-line-error
PRE =  $(TEX) -ini -job-name="preamble" "&pdflatex preamble.tex\dump"
BIB = bibtex

.PHONY: all view

all : lin-prog-main.pdf

view :
	open lin-prog-main.pdf

lin-prog-main.pdf : lin-prog-main.tex lin-prog-main.bbl lin-prog-main.blg 
	$(TEX) lin-prog-main.tex

lin-prog-main.bbl lin-prog-main.blg : lin-prog-main.aux bib.bib 
	$(BIB) lin-prog-main

lin-prog-main.aux : lin-prog-main.tex
	$(TEX) lin-prog-main.tex

lin-prog-main.bib : lin-prog-main.tex
	$(TEX) lin-prog-main.tex

#preamble.fmt : preamble.tex
	$(PRE) prea`mble.tex


clean :
	rm *.aux *.toc *.log *.out *.snm *.nav *.tex.backup *.synctex.gz main.pdf



